Grounded Objects and Interactions for Video Captioning

We address the problem of video captioning by grounding language generation on object interactions in the video. Existing work mostly focuses on overall scene understanding with often limited or no emphasis on object interactions to address the problem of video understanding. In this paper, we propose SINet-Caption that learns to generate captions grounded over higher-order interactions between arbitrary groups of objects for fine-grained video understanding. We discuss the challenges and benefits of such an approach. We further demonstrate state-of-the-art results on the ActivityNet Captions dataset using our model, SINet-Caption based on this approach.

==> sections/acknowledgement.tex <==
\section*{Acknowledgments}
Zsolt Kira was partially supported by the National Science Foundation and National Robotics Initiative (grant \# IIS-1426998).

==> sections/impl.tex <==
\section{Dataset and Implementation} 
% \subsection{Datasets:}
\textbf{ActivityNet Captions dataset:}
We use the new ActivityNet Captions for evaluating \netshort.  
% To evaluate \netshort\ on a sequence-to-sequence problem for video, we use ActivityNet Captions for video captioning. 
% The ActivityNet Captions dataset contains 20k videos and has total 849 video hours with 100k total descriptions. 
% Although the number of videos is less compared to Kinetics, the video hours is in fact slightly longer than Kinetics (approximately 833 hours).
We focus on providing the fine-grained understanding of the video to describe video events with natural language, as opposed to identifying the temporal proposals. 
We thus use the ground truth temporal segments and treat each temporal segment independently. 
% We use this dataset over other captioning datasets because ActivityNet Captions is action-centric, as opposed to object-centric~\cite{krishna2017dense}. 
% This fits our goal of detecting higher-order object interactions for understanding human actions.
% Following the same procedure as in \cite{krishna2017dense}, all sentences are capped to be a maximum length of 30 words. 
We sample predictions using beam search of size 5 for captioning. 
While the previous work sample C3D features every 8 frames~\cite{krishna2017dense}, we only sampled video at maximum 1 FPS. Video segments longer than 30 seconds are evenly sampled at maximum 30 samples. 

% \subsection{Implementation Details:}
% We now discuss how to extract image and object features for ActivityNet Captions. 

\textbf{Image feature:}
We pre-trained a ResNeXt-101 on the Kinetics dataset~\cite{kay2017kinetics} sampled at 1 FPS (approximately 2.5 million images), and use it to extract image features.
% We use SGD with Nesterov momentum as the optimizer. 
% The initial learning rate is $1e-4$ and automatically drop by 10x when validation loss saturated for 5 epochs. 
% The weight decay is $1e-4$ and the momentum is 0.9, and the batch size is 128. 
% We follow the standard data augmentation procedure by randomly cropping and horizontally flipping the video frames during training. 
% When extracting image features, the smaller edge of the image is scaled to 256 pixels and we cropped the center of the image as input to the fine-tuned ResNeXt-101.
Each image feature is encoded to a 2048-d feature vector. 

\textbf{Object feature:}
We generate the object features by first obtaining the coordinates of ROIs from a Deformable R-FCN~\cite{dai2017deformable} (pre-trained on MS-COCO) with ResNet-101~\cite{he2015deep} as backbone architecture. 
% The Deformable R-FCN was trained on MS-COCO train and validation dataset~\cite{lin2014microsoft}. 
We set the IoU threshold for NMS to be 0.2. 
For each of the ROIs, we extract features using ROI coordinates and adaptive max-pooling from the same ResNeXt-101 model pre-trained on Kinetics. 
% Using the ROI features obtained from Deformable R-FCN only has minor affect when trained with image features. 
The resulting object feature for each ROI is a 2048-d feature vector. 
ROIs are ranked according to their ROI scores. We select top 15 objects only. 
% Note that we have various number of ROIs for each video frame, and video length can also be different.  
% We do not use object class information since there is a cross-domain problem and we may miss some objects that were not detected.
% For the same reason, the bounding-box regression process is not performed here since we do not have the ground-truth bounding boxes.

\textbf{Training:}
We train the proposed \netshort\ with ADAM optimizer. 
The initial learning rate is set to $1e-3$ and automatically drop by 10x when validation loss is saturated. 
The batch sizes is $32$. 


==> sections/ref.tex <==
\section*{References}

References follow the acknowledgments. Use unnumbered first-level
heading for the references. Any choice of citation style is acceptable
as long as you are consistent. It is permissible to reduce the font
size to \verb+small+ (9 point) when listing the references. {\bf
  Remember that you can go over 8 pages as long as the subsequent ones contain
  \emph{only} cited references.}
\medskip

\small

[1] Alexander, J.A.\ \& Mozer, M.C.\ (1995) Template-based algorithms
for connectionist rule extraction. In G.\ Tesauro, D.S.\ Touretzky and
T.K.\ Leen (eds.), {\it Advances in Neural Information Processing
  Systems 7}, pp.\ 609--616. Cambridge, MA: MIT Press.

[2] Bower, J.M.\ \& Beeman, D.\ (1995) {\it The Book of GENESIS:
  Exploring Realistic Neural Models with the GEneral NEural SImulation
  System.}  New York: TELOS/Springer--Verlag.

[3] Hasselmo, M.E., Schnell, E.\ \& Barkai, E.\ (1995) Dynamics of
learning and recall at excitatory recurrent synapses and cholinergic
modulation in rat hippocampal region CA3. {\it Journal of
  Neuroscience} {\bf 15}(7):5249-5262.

==> sections/related.tex <==
\section{Related work}
We discuss existing work on video understanding based on video captioning as well as related work on detecting visual relationships in images and videos.

\textbf{Video captioning:}
Similar to other video tasks using deep learning, initial work on video captioning learn compact representations combined over time. This single representation is then used as input to a decoder, e.g. LSTM, at the beginning or at each word generation to generate a caption for the target video~\cite{pan2016jointly, venugopalan2015sequence, venugopalan2014translating}. 
Other work additionally uses spatial and temporal attention mechanisms to selectively focus on visual content in different space and time during caption generation~\cite{song2017hierarchical,  yao2015describing, yu2016video}. 
Similar to using spatial attention during caption generation, other work has additionally incorporated semantics attributes~\cite{gan2016semantic, pan2016video, shen2017weakly, yu2017end}. 
However, these semantic or attribute detection methods with attention or non-attention mechanisms do not consider object relationships and interactions, i.e. they treat the detected attributes as a bag of words. 
Our work, \netshort-Caption\ uses higher-order object relationships and their interactions as visual cues for caption generation. 

\textbf{Interactions/Relationships in images:}
%Previous works have used relationship between objects to improve object recognition performance~\cite{galleguillos2008object, gould2008multi}. This contrasts with our goals of learning relationships and improving video understanding using existing object detection methods. %
%Pre-deep learning relationships work that are highly-cited: ~\cite{maji2011action, rohrbach2013translating, yao2010modeling}
Recent advances in detecting visual relationships in images use separate branches in a ConvNet to explicitly model object, human, and their interactions~\cite{chao2017learning, gkioxari2017detecting}.
Visual relationships can also be realized by constructing a scene graph which uses a structured representation for describing object relationships and their attributes~\cite{johnson2015image, li2017scene, liang2017deep, xu2017scene}.
Other work on detecting visual relationships explore relationships by pairing different objects in the scene~\cite{dai2017detecting, hu2016modeling, santoro2017simple, zhang2017visual}. 
While these image based models can successfully detect visual relationships for images, a scene with many objects may have only a few individual interacting objects. 
It would be inefficient to detect all relationships across all individual object pairs~\cite{zhang2017relationship}. 
This problem becomes even more severe in videos, making these methods intractable. 

\textbf{Interactions/Relationships in video:}
Compared to the image domain, there is limited work in exploring relationships for fine-grained video understanding.
Ni et al.~\cite{ni2014multiple} use a probabilistic graphical model to track interactions, but their model 
% can only handle the binary contextual relationship between objects.
% which considered mutual geometrical relationship
% This method 
is insufficient to model interactions involve multiple objects.
To overcome this issue, Ni et al.~\cite{ni2016progressively} propose using a set of LSTM nodes to incrementally refine the object detections. 
% In contrast, Lea et al.~\cite{lea2016segmental} propose to decompose the input image into several spatial units in a feature map, which then captures the object locations, states, and their 
relationships using shared ConvNets. 
However, limited by the availability of an appropriate dataset, these existing works focus on indoor or cooking settings where the human subject along with the objects being manipulated are at the center of the image.
Also, their methods can only handle pairwise relationships between objects. Yet, human action can be complex and often involve higher-order object interactions. 
Therefore, \netshort\ attentively models object inter-relationships and discovers the higher-order interactions on large-scale, open domain, and fine-grained video understanding problem. 

